Robust Inference in Panel Data Models: Some Effects of Heteroskedasticity and Leveraged Data in Small Samples

With the violation of the assumption of homoskedasticity, least squares estimators of the variance become inefficient and statistical inference conducted with invalid standard errors leads to misleading rejection rates. Despite a vast cross-sectional literature on the downward bias of robust standard errors, the problem is not extensively covered in the panel data framework. We investigate the consequences of the simultaneous presence of small sample size, heteroskedasticity and data points that exhibit extreme values in the covariates ('good leverage points') on the statistical inference. Focusing on one-way linear panel data models, we examine asymptotic and finite sample properties of a battery of heteroskedasticity-consistent estimators using Monte Carlo simulations. We also propose a hybrid estimator of the variance-covariance matrix. Results show that conventional standard errors are always dominated by more conservative estimators of the variance, especially in small samples. In addition, all types of HC standard errors have excellent performances in terms of size and power tests under homoskedasticity.

==> mc_simul2_old.tex <==

%%het
%beta1
\par Under heteroskedasticity, results differ across simulation designs for the contaminated variable.
\par \textbf{Simulation 1.} Looking at Table~\ref{tab:simul1_v1}, PHC0 standard errors considerably underestimate the ``true'' standard error, with a $PB>20\%$, for different combinations of $\{N,T\}$ that yield to a an overall panel size of $n<2500$, and also produce test statistics taht are upward distorted, as expected. PHC6 standard errors are also upward biased in small samples leading to the over-rejection of the true null hypothesis but not as often as PHC0 does. However, as the sample size increases the former tends to mimic the behaviour of the two most conservative estimators, PHC3 and PHCjk, in terms of probability bias and rejection probability. Standad errors obtained with PHC3 and PHCjk formulae are much less biased than the other two alternatives, although their size is slightly distorted downwards but still the closest to the nominal $5\%$ level when $n<2500$. Despite the upward bias of PHC0 that persists in large samples, its empirical size is the closest to the nominal level of 5\% for different combinations of $\{N,T\}$ that yield to a an overall panel size of $n\ge2500$. 
\par \textbf{Simulation 2.} With unbalaced panel data and correlation between the regressor and the unobserved heterogeneity, results for simulation of type 2 in Table~\ref{tab:simul2_v1} are in strack contrast with respect to those obtained for simulation of type 1 as PHC3, PHC6 and PHCjk always improve upon PHC0. In particular, PHC3 and PHCjk standard errors have a low proportional bias and their test statistics show small size distortions that well approximate the canonical $5\%$-level. Although PHC6 imitates PHC0's behaviour for $N=25$ and all $T$, its performance converges towards PHC3 and PHCjk's as the sample increases.
%beta2
\par Similar results are obtained for the uncontaminated variable under heteroskedasticity as shown in  Tables~\ref{tab:simul1_v2} and \ref{tab:simul2_v2}.
\par \textbf{Simulation 1.} PHC0 standard errors outperform all other estimators of the variance even though they display a greater (positive) bias but the empirical size of their test statistics is the closest to the nomial level, especially compared to those compited using PHC3 and PHCjk standard errors whose rejection probabilities touch 0\% with $N=\{25,50\}$ and for all $T$. On the other hand, PHC6 estimator performs almost as well as the conventional robust formula with $T=20$ and for all $N$. As the panl sample size increases, the rejection probabilities of PHC3, PHC6 and PHCjk standard errors tend to converge to the same value and, despite their smaller proportional bias, PHC0 test statistics have the most accurate empirical size.
 \par\textbf{Simulation 2.} These considerations remain valid for simulation design of type 2. The additional note to point out is that among the three alternative standard error formulae, PHC6 formula always displays better performances in terms of proportional bias and empirical size than  PHC3 and PHCjk.


%\par Under heteroskedasticity,  PHC0 generates test statistics that are, as expected, significantly over-sized when the variable is contaminated with leverage points, showing the same downward pattern towards the selected test size as $N$ increases keeping $T$ fixed. The over-rejection probability is much higher compared to the homoskedastic case. Conversely,  PHC0 test statistics tend to slightly  under-reject the null hypothesis  without leveraged data whereas size distortions are particularly evident for PHC3 and PHC$jk$ (Panel B in Figure~\ref{fig:size5}). Unlike these conservative estimators that tend to under-reject the null hypothesis at almost 0\%,  PHC6 test statistics are not that undersized but show an upward movement towards PHC0 raw sizes, especially as the sample size increases fixing the time length. 
%\par Overall, we observe that  PHC6 test statistics tend not to be upward biased as those computed with PHC0 formula in small samples (Figure~\ref{fig:size1} and Panel A in Figure~\ref{fig:size5}) but not as distorted downwards as the most conservative estimators  (Panel B in Figure~\ref{fig:size5}). 



%%homo

%beta1
\par Under homoskedasticity, similar conclusions can be drawn by looking at the results for the slope coefficient of the contaminated variable from Tables~\ref{tab:simul1_v1homo} and \ref{tab:simul2_v1homo}.
\par \textbf{Simulation 1 and 2.} PHC3 and PHCjk estimators have better performances in terms of empirical size and proportional bias than PHC0 standard errors that understimate the true variance and over-reject the null hypothesis in almost all combinations of $\{N,T\}$. PHC6 performs much better than the first two when $N\ge50$ and for all time periods, instead. In spite of having the smaller bias in absolute value, the empirical size of PHC6 test statistics tends to be slightly distorted upwards compared to  PHC3 and PHCjk. As the sample size increases above 2500 units (for different combinations of  $\{N,T\}$) PHC0 shows a decent behaviour.
%beta2
\par Unlike the case above, results under homoskedasticity differ across simulations for the uncontaminated variable.
\par \textbf{Simulation 1.} From Table~\ref{tab:simul1_v2homo}, PHC0 and PHC6 outperform the other two estimators in terms of rejection probabilities and, among the two, PHC6 is less upward biased with empirical size closer to $5\%$. Despite the smaller bias of PHC3 and PHCjk standard errors, their size is distorted downwards but as the smaple size increases, their size approxiamtes the nomial significance level with a smaller probability bias.
 \par\textbf{Simulation 2.} All estimators show a good overall performance in Table~\ref{tab:simul2_v2homo} but PHC6 excells in  almost all combinations of $\{N,T\}$. In particular, for $T=5$ PHC6 outperforms the other estimators for having both a small proportional bias and a suitable empirical size. Even though  PHC3 and PHCjk behave as well as PHC6 in terms of rejection probabilities, they have on average a higher proportional bias in absolute value. Overall, PHC0 does not perform extremely poorly.
%\par  In the absence of heteroskedasticity and independently of the degree of contamination, PHC0 test statistics tend on average to over-reject the true null hypothesis when the panel size is small, i.e., $N<1000$,  displaying a gradual downward movement towards 5\% as the sample size increases with PHC6 resembling this descending pattern. The rejection rate is higher under contamination ($\beta_1$) compared to lack of contamination in the variables ($\beta_5$). Tests based on  the most conservative estimators PHC3 and PHC$jk$ estimators tend to  outperform PHC0 for $N<1000$ and for all $T$ as their empirical size is close to the correct size independently of the degree of contamination, \emph{ceteris paribus}. This suggests that the use of PHC3 and PHC$jk$ formulae may contribute to enhance inference even in the absence of heteroskedasticity, \emph{ceteris paribus}. 
%

==> tex_files/app_stata.tex <==
\section{A New Stata Command: \texttt{xtfe}}
Simulation results in Section~\ref{sec:simulres} and the empirical examples in Section~\ref{sec:examples} have been obtained using the authored-written command \texttt{xtfe} in \textsc{stata}.
\par The \texttt{xtfe} command fits fixed-effects (FE) models allowing for the choice of various versions of heteroskedasticity-consistent standard errors. Its syntax is as follows

\noindent \texttt{xtfe \emph{depvar} [\emph{indepvars}] [if] [in] [weight], [, \underline{l}evel(\#)  vce(\emph{\textcolor{blue}{vcetype}})]}

%\begin{adjustwidth}{1cm}{2cm}
\texttt{
\textbf{\underline{l}evel(\#)}   \hspace{.5cm}       set confidence level; default is level(95) \\
\textbf{vce(\emph{\textcolor{blue}{vcetype}})}     \emph{vcetype} may be conventional (if no vcetype is specified), \underline{r}obust, phc3, phc6, \underline{jack}knife \underline{fig}ure
}
%\end{adjustwidth}

\par  \texttt{xtfe} reproduces the outcome of \textsc{stata's} \texttt{xtreg} for FE models but gives two additional choices of heteroskedasticity-consistent standard errors:  \texttt{phc3} and \texttt{phc6}. The command has been adapted to support unbalanced data, factor variables, and time series variables. 
\par The option \texttt{\underline{fig}ure} plots the demeaned residuals over the fitted values to detect any form of heteroskedasticity.

\


\section{A New Stata Command: \texttt{xtlvr2plot}}
\section{A New Stata Command: \texttt{pddiagnostics2}}



==> tex_files/model3_Ti.tex <==
\section{Model and Assumptions}\label{sec:model}
%new version
\noindent Consider the static linear panel regression model with one-way error component
\begin{equation}\label{eq:fe}  
\y =  \x' \bm{\beta} + \alpha_i + \error, \hspace{5pt}  i \in \mathcal{I}=\{1,\dots,N\} \hspace{3pt}  \text{and} \hspace{3pt}  t\in \mathcal{T}=\{1,\dots,T_i\}
\end{equation}
% i= 1,\dots, N, \hspace{3pt}  t= 1,\dots, T_i
where $\y$ is the response variable for the cross-sectional unit $i$ at time period $t$; $\x$ is a $k\times1$ vector of time-varying inputs, $\bm{\beta}$ is a $k\times1$ vector of parameters of interest; $\alpha_i$ is the individual-specific unobserved heterogeneity (or \emph{fixed effects}); and $\error$ is a stochastic error component. We consider a framework where the panel is small, that is, the time period length is smaller than the number of units $N$ such that $T_i \ll N$, with $T_i\le T$ for all $i$. Under this notation $T$ is the full set of time information while $T_i<T$ denotes that some data are missing for unit $i$ and, therefore, the panel is unbalanced. In the case of unbalanced panel data, the total number of observations in the sample is  given by $n = \sum_{i=1}^{N}T_i$ whereas  $n = N\cdot T$ with balanced data sets. When $T=2$ and only one period is observed for the $i$th unit, $T_i=1$, the $i$th unit is treated as a cross-section.
%and $\error$ is a one-way composite stochastic that incorporates with an individual-specific unobserved heterogeneity, $\alpha_i$, and the idiosyncratic error, $\epsit$.
%%%%
\par Stacking observations for $t$, model \eqref{eq:fe} at the level of the observation becomes
 \begin{equation}\label{eq:fe_i}   
\yii =   \xii\bm{\beta} +\bm{\alpha}_i+ \errori,  \,\,\, \text{for all}  \,\,\, i= 1,\dots, N, 
\end{equation}
\noindent where $\yii$ is $T_i\times1$ vector of outcomes; $\xii$ is a $T_i\times k$ matrix of regressors; $\bm{\alpha}_i=\alpha_i\iotat$ is a $T_i\times1$ vector of individual fixed effects, and $\iotat$ is a vector of ones of order $T_i$; and $\errori$ is a $T_i\times1$ vector of one-way error component.  
%This  formulation allows for  models that either include a random  individual-specific component, independent of the observables, in the compound error \footnote{In models with random effects, the one way error term is defined as the sum of two vector components $\epsi$ and $\bm{\alpha}_i$, where individual fixed-effect is $\bm{\alpha}_i=\iotat\alpha_i$, and $\iotat$ is a vector of ones}
%\par Under the assumption \mbox{$\E(\bm{\alpha}_i|\xii)=h(\xii)$}, the parameter of interest $\bm{\beta}$ can be consistently estimated applying an appropriate transformation to the data, i.e., \emph{time-demeaning} or \emph{first-differencing} the original model. 
\par The fixed effects $\bm{\alpha}_i$ in Equation~\eqref{eq:fe_i} are removed by consistently estimating the parameter of interest $\bm{\beta}$ via an appropriate transformation of the original data, i.e., the \emph{time-demeaning} or \emph{first-differencing} procedure, because it might be the case that \mbox{$\E(\bm{\alpha}_i|\xii)=h(\xii)$}. In the following discussion, we exclusively focus on the first approach when applied to model~\eqref{eq:fe_i}, such that the estimating equation becomes
%%%%%
 \begin{equation}\label{eq:fe_wg_i}   
\yi =  \Xii\bm{\beta} + \uii, \,\,\, \text{for all}  \,\,\, i= 1,\dots, N,  
\end{equation}
\noindent where $\yi=(\I_{T_i}-\, T_i\inv\iotat\iotat')\yii$ is $\Ti\times1$; $\Xii=(\I_{\Ti}-\, \Ti\inv\iotat\iotat')\xii$ is $\Ti\times k$; and $\uii=(\I_{\Ti}-\, T_i\inv\iotat\iotat')\errori$ is $\Ti\times1$. Note that $(\I_{\Ti}-\, \Ti\inv\iotat\iotat')\bm{\alpha}_i=\zero$ as $\Ti\inv \iotat\iotat' \bm{\alpha}_i=\bm{\alpha}_i$.  The aforementioned data transformation delivers a consistent estimator of $\bm{\beta}$ even when the regressor is correlated with the unobserved heterogeneity $\alpha_i$, but is less efficient than the First-Difference (FD) transformation with errors that are not identically distributed. The  within-group estimator is the Pooled OLS estimator of Equation~\eqref{eq:fe_wg_i}. 
%\par Henceforth, we state the model assumptions and estimator's properties in terms of the variables $\yii$, $\xii$ and $\errori$ that in models with unobserved heterogeneity can be interpreted as random variables whose data transformation removed the presence of the individual-specific fixed effects from the equation, as mentioned above. 

\par  The model assumptions are as follows
%%%
\begin{enumerate}[label=\sc{A.}{\arabic*}, leftmargin=1.7\parindent,  rightmargin=.5\parindent]
\item (\emph{data-generating process}): \label{item:dgp} %%
 	\begin{enumerate}[label={\roman*)}]
	\item  $\{\xii\}$ is an independent and identically distributed (\emph{iid}) sequence of random variables, for all $\, i = 1, \dots, N$; \label{item:dgp_x}
	\item $\{\errori\}$ is an independent  but not identically distributed (\emph{inid}) sequence of random error terms, for all $\, i = 1, \dots, N$.  \label{item:dgp_u}
	\end{enumerate}
	

\item (\emph{on the relation of $\Xii$ and $\uii$}):\label{item:xu}
 	\begin{enumerate}[label={\roman*)}]
	\item (\emph{strong exogeneity}): $\E\bigl(\uii|\Xii\bigr)=0$, for all $i= 1,\dots, N$; \label{item:exogeneity}
	\item  (\emph{heteroskedasticity}): $\bSgma=N\inv \sum_{i=1}^N\Sgma\to\Ssgma$, where the  matrix of the heteroskedastic disturbances $\Sgma=\E\bigl(\uii\uii'|\Xii\bigr)= \mathrm{diag}\bigl\{\sigma_{it}^2\bigr\}$ is  symmetric  of dimension $T_i$, finite, positive definite, and diagonal. \label{item:het}
	\end{enumerate}
%with diagonal \mbox{elements $\sigma^2_{it}$} and zero elsewhere
	\end{enumerate}

%Ass. explanation
\par The above model assumptions have the following implications. \ref{item:dgp}.\ref{item:dgp_x} guarantees that the sequence of random variables $\{\xii' \xii \}$ is \emph{iid} [\textsc{prop 3.3} in \citet[p.30]{white1984}]. \ref{item:dgp}.\ref{item:dgp_u} imposes cross-sectional independence and, together with \ref{item:dgp}.\ref{item:dgp_x}, implies that $\{\xii' \errori \}$ is an \emph{inid} sequence of random vectors [\mbox{\textsc{prop 3.10}} in \citet[p.34]{white1984}]. Assumption \ref{item:dgp} and its implications remain unaltered after any data transformation.
%
%An implication of \ref{item:1way_error}  is $\error|\xii\distas{}NID(0,\sigma^2_{it})$, where $\sigma^2_{it}= \sigma^2_{\alpha}+\sigmaeps$.
%
\par The strict exogeneity assumption \ref{item:xu}.\ref{item:exogeneity} rules out feedback effects and implies contemporaneous exogeneity, i.e., $\E\bigl(\tildeuit|\Xii\bigr)= \E\bigl(\tildeuit|\xit \bigr)=0$, and is a crucial assumption to prove consistency of the \emph{within-group} estimator. The projection analog of \ref{item:xu}.\ref{item:exogeneity}  is the strong exogeneity condition, i.e, $\E\bigl(\widetilde{\mathbf{x}}_{is}\tildeuit)=0 \Leftrightarrow \E\bigl(\tildeuit|\Xii\bigr)\mbox{=0}$, for all $s\in \mathcal{T}$ and $s\ne t$. Assuming the exogeneity of the undemeaned variables might not be strong enough to guarantee that exogeneity is preserved \emph{after} the time-demeaning transformation\footnote{\red{This occurs because the regressor might be correlated with $T_i\inv\iotat\iotat'\uii$ since it includes the whole history.}}, i.e., $\E\bigl(\xii'\errori\bigr)\mbox{=0} \not\Rightarrow  \E\bigl(\Xii'\uii\bigr)\mbox{=0}$ \citep[p.707]{cameron2005}.  %The assumption is an implication of  \ref{item:1way_error} such that $\E(\error|\xii)=\E(\alpha_i|\xii)+\E(\epsit|\xii)=0$.
%
Assumption  \ref{item:xu}.\ref{item:het} allows the conditional error variance to vary across observations and time periods, and  imposes serial uncorrelation over time dimension, $\E\bigl(\tildeuit \widetilde{u}_{is}|\Xii\bigr)=0$ with $ (t,s)\in \mathcal{T}$ and $ t \ne s$. 


\par The assumptions for the existence and optimality properties of the estimator of the true population parameter $\bm{\beta}$ are 

\begin{enumerate}[label=\sc{A.}{\arabic*}, leftmargin=1.7\parindent, rightmargin=.5\parindent]
\setcounter{enumi}{2}
\item (\emph{rank condition}): $\Sxx \equiv N\inv \sum_{i=1}^N \Xii'\Xii$ is a finite symmetric matrix with full column rank $k$. \label{item:rank}

\item (\emph{moment conditions}):  \label{item:mom} %%
 	\begin{enumerate}[label={\roman*)}]		
 	 	\item  $\E\big\|\Xii'\Xii\big\|<\infty$ for  $\Xii'\Xii\in \mathbb{R}^{k\times k}$;  \label{item:mom_x2} 			
 	 	\item  $\mathrm{sup}_{i}\,\E\big\|\Xii' \uii\big\|^{2+\delta}<\infty$ for some $\delta>0$, $\forall i$ and $\Xii' \uii \in \mathbb{R}^k$, \label{item:mom_Adistr}	%uniform mom bound
	\end{enumerate}	
 \noindent where $\|\cdot\|$ denotes the Euclidean norm.

\item  (\emph{average variance-covariance matrix convergence}): \label{item:V} \\
$\bVn=N\inv \sum_{i=1}^N \, \Vi\to\Vv$, where $\Vi=\E\bigl(\Xii'\Sgma\Xii\bigr)$ and $\Vv$ is a finite positive definite $k\times k$ matrix.
\end{enumerate}

%Ass. explanation
The full column rank condition in \ref{item:rank} implies non-singularity of the matrix $\Sxx$ and, hence, no perfect multicollinearity that guarantees the invertibility of the matrix.  The limiting matrix $\SSxx \equiv \E\bigl(\Xii'\Xii\bigr)$ possesses the properties of $\Sxx$ by the \emph{Weak Law of Large Numbers} (\emph{WLLN}) [\mbox{\textsc{thm 6.6}}.  Another implication of \ref{item:rank} is that the matrix of regressors $\Xii$ is full column rank.
%
%
\mbox{Assumption \ref{item:mom}} defines the finiteness and boundedness of moments in terms of the Euclidean norm. 
%
Assumption \eqref{item:V} ensures that the average variance-covariance matrix converges to a finite quantity, satisfying one of the conditions of the \emph{Multivariate Central Limit Theorem} (\emph{MCLT}) for \emph{inid} processes  [\textsc{thm 6.16} in \citet[p.189]{hansen2019}].
%
%
%Within individual correlation is presen to get a consistent estimator as \citet{arellano1987} and \citet{stock2008} suggest. 
\par  No restrictions are placed on influential points, i.e., high leverage points and outliers\footnote{With high leverage points, we identify those anomalous observations that appear to be isolated from the main body of points in the space of the covariates as they assume extreme values, but follow the same trend of the rest of the data \citep[p.140]{chatterjee1986, greene2012}, whereas outliers are points in the response-factor space with large squared normalised residual following the opposite trend of the cloud of data points, and lying far from the regression line \citep[p.141]{chatterjee1986, greene2012}.}; here, we possibly allow for their presence.
\par This set of assumptions and their implications remain valid under any monotonic data transformation due to the \emph{Continuous Mapping Theorem} (\emph{CMT}) [\textsc{thm 6.19} in \citet[p.192]{hansen2019}]. Later in this work, we consider the \emph{within-group} transformation of the data. 

\section{Asymptotic Properties of $\beta$}\label{sec:properties}


 Under \ref{item:dgp}--\ref{item:mom}.\ref{item:mom_x2}, the \emph{the within-group} estimator of the true population parameter $\bm{\beta}$ exists with form $\bfen= \Bigl(N\inv \sum_{i=1}^N \Xii'\Xii \Bigr)\inv \,\, N\inv\sum_{i=1}^N  \Xii'\yi$, and is consistent, i.e.,
\begin{equation}\label{eq:bfe_asymptotic}
\bfen -  \bm{\beta} = \Biggl(\frac{1}{N} \sum_{i=1}^N \Xii'\Xii \Biggr)\inv \,\, \frac{1}{N} \sum_{i=1}^N \Xii\uii \overset{p}{\to}\bm{0} \,\,\, \mathrm{as} \,\,\,N\to \infty.
\end{equation}

%\begin{addmargin}[3em]{3em}
%Proof existence & consistency
%block A: X'X
By the previously discussed implication of \ref{item:dgp}.\ref{item:dgp_x} and \textsc{prop 3.3} in \citet[p.30]{white1984}, $\bigl\{\Xii'\Xii\bigr\}$ is an \emph{iid} sequence of random variables with finite moments given \ref{item:mom}. The elements of the sequence satisfy the \emph{Weak Law of Large Numbers} (\emph{WLLN}) [\mbox{\textsc{thm 6.6}} in \citet[p.182]{hansen2019}] such that \mbox{$\Sxx \overset{p}{\to} \SSxx<\infty$}. Because both matrices are invertible by \ref{item:rank}, then \textsc{thm 6.19} [\emph{Continuous Mapping Theorem (CMT)} in \citet[p.192]{hansen2019}] yields the result \mbox{$\Sxx\inv \overset{p}{\to} \SSxx\inv$}. 
%block B: X'u
Now, we want to show that the second component in \eqref{eq:bfe_asymptotic} converges in probability to zero. We know that the sequence $\bigl\{\Xii'  \uii\bigr\}$ is \emph{inid} as an implication of \ref{item:dgp} [\textsc{prop 3.10} in \citet[p.33]{white1984}]. Then, the Chebyshev inequality is
\begin{equation}\label{eq:chebyshev}
\mathrm{Pr}\Biggl(\Bigg\| \frac{1}{N} \sum_{i=1}^N \Xii' \uii\Bigg\|\ge \epsilon\Biggr) \le \frac{\E\Big\|\frac{1}{N} \sum_{i=1}^N \Xii' \uii \Big\|^2}{\epsilon^2},
\end{equation}

%%%%%
\noindent where the numerator in \eqref{eq:chebyshev} can be expanded as follows
\begin{equation}\label{eq:induced_norm}
\begin{split}
\Bigg\|\frac{1}{N} \sum_{i=1}^N \Xii' \uii \Bigg\|^2 & = \tr\Biggl\{\Biggl(\frac{1}{N} \sum_{i=1}^N   \Xii'\uii\Biggr) \, \Biggl(\frac{1}{N} \sum_{j=1}^N \errorj'\xij\Biggr) \Biggr\}\\
& = \frac{1}{N^2}\, \tr\Biggl\{\sum_{i}\sum_{j}  \Xii'\uii\errorj'\xij\Biggr\}.
\end{split}
\end{equation}
\noindent By the aforementioned implication of \ref{item:dgp}.\ref{item:dgp_u} and under \ref{item:xu}.\ref{item:het} the conditional error variance is
\begin{equation}\label{eq:system}
\E\bigl(\Xii'\uii\errorj'\xij\big| \Xii \xij\bigr) = 
\begin{cases}
0 & \forall i \ne j\\
\Xii'\Sgma\Xii &\forall i= j
\end{cases}
\end{equation}
%\par Set  the average variance-covariance matrix $\bVn=N\inv\sum_{i=1}^N\Vi$, where  $\Vi=\E\bigl(\xii'\Sgma\xii\bigr)$  is a finite, symmetric and positive definite matrix by construction.  The matrix $\bVn$ has the properties of $\Vi$. Let $\lambda_l(\bVn)$ be the $l\th$ eigenvalue of $\bVn$. 
\par Applying the expected value operator to \eqref{eq:induced_norm}, and using result \eqref{eq:system} jointly with the \emph{Law of Iterated Expectations} (LIE), the above equality becomes as follows
\begin{equation}\label{eq:exp_induced_norm}
\begin{split}
\E\Bigg\|\frac{1}{N} \sum_{i=1}^N \Xii' \uii \Bigg\|^2 & = \frac{1}{N^2}\, \tr\Biggl\{\sum_{i}\sum_{j} \, \E\bigl(\Xii'\uii\errorj'\xij\bigr)\Biggr\} \\
& = \frac{1}{N^2}\, \tr \Biggl\{\sum_i\sum_j \, \E\Bigl(\E\bigl(\Xii'\uii\errorj'\xij\big| \Xii \xij\bigr)\Bigr)\Biggr\} \\
& = \frac{1}{N^2}\, \tr \Bigl\{\sum_i \, \E\bigl(\Xii'\Sgma\Xii \bigr)\Bigr\} \\
& = \frac{1}{N}\, \tr \biggl\{ \frac{1}{N}\sum_i \, \E\bigl(\Xii'\Sgma\Xii \bigr)\biggr\} \\
& = \frac{1}{N}  \tr \bigl\{\bVn\bigr\} \to 0, \hspace{2mm} \mathrm{as} \,\, N \to \infty
%& = \frac{1}{N} \sum_{l=1}^K \lambda_l(\bVn)\\
%& \to 0 \,\,\,\, \mathrm{as} \,\, N \to \infty,
\end{split}
\end{equation}
\noindent  since assumption \eqref{item:V} implies that $ \tr \bigl\{\bVn\bigr\} \to \tr \bigl\{\Vv\bigr\} $, which is finite. 
\par We showed that the right-hand side of equality \eqref{eq:exp_induced_norm} converges in probability to zero, so does the left-hand side. Inequality \eqref{eq:chebyshev} becomes

\begin{equation*}
\mathrm{Pr}\Biggl(\Bigg\| \frac{1}{N} \sum_{i=1}^N \Xii' \uii\Bigg\|\ge \epsilon\Biggr)\to 0 \,\,\,\, \mathrm{as} \,\, N \to \infty,
\end{equation*}
\noindent and, hence, $N\inv  \sum_i\Xii'\uii\overset{p}{\to} \bm{0}$.
%blocks A&B
\noindent By \textsc{thm 6.19} [CMT in \citet[p.192]{hansen2019}] , the result follows $\bfen - \bm{\beta} \overset{p}{\to} \SSxx\inv \cdot \bm{0} = \bm{0}$, or alternatively $\bfen \overset{p}{\to} \bm{\beta}$. However,  this result holds for any monotonic transformation of the data, e.g., the within-group transformation. %Using \textsc{thm 6.19} again, we get the wanted result $\tbfen \overset{p}{\to} \bm{\beta}$.
%\end{addmargin}

\

Under  \ref{item:dgp}--\ref{item:V}, the estimator has asymptotic distribution 
\begin{equation}\label{eqn:avar}
\sqrt{N}\bigl(\bfen - \bm{\beta}\bigr) \overset{d}{\to}\N \bigl(\bm{0},\SSxx\inv \Vv\SSxx\inv\bigr)\hspace{4mm} \mathrm{as} \,\, N \to \infty.
%\sqrt{N}\bigl(\bfen - \bm{\beta}\bigr) = \Biggl(\frac{1}{N} \sum_{i=1}^N \Xii'\Xii \Biggr)\inv \,\, \frac{1}{\sqrt{N}}\sum_{i=1}^N  \Xii'\uii  \overset{d}{\to}\N\bigl(\bm{0}, \SSxx\inv\Vi\SSxx\inv\bigr).
\end{equation}

% Proof Avar
%\begin{addmargin}[3em]{3em}
Rewrite the LHS of Equation~\ref{eqn:avar} as follows
%%%%%%%%%%%%%%%%%%%%%
\begin{equation*}
\small
\sqrt{N}\bigl(\bfen - \bm{\beta}\bigr) = \Biggl(\frac{1}{N} \sum_{i=1}^N \Xii'\Xii \Biggr)\inv \,\, \frac{1}{\sqrt{N}}\sum_{i=1}^N  \Xii'\uii.
\end{equation*}
%%%%%%%%%%%%%%%%%%%%%
%block A: X'X
The sequence of random variables $\bigl\{\Xii'\Xii\bigr\}$ is \emph{iid} as implication of \ref{item:dgp}.\ref{item:dgp_x} and by \textsc{prop 3.3}  in \citet[p.30]{white1984}. With analogous arguments as those used above to prove consistency, $\Sxx\inv \overset{p}{\to} \SSxx\inv$. 
%block B: X'u
Under assumptions \ref{item:dgp} and \ref{item:xu}.\ref{item:exogeneity} and by \textsc{prop 3.10} in \citet[p.33]{white1984}, the sequence $\bigl\{\Xii'  \uii\bigr\} \in \R^k$ is \emph{inid} with means $\E\bigl(\Xii'\uii \bigr)=0$ and variance matrices \mbox{$\Vi=\E\bigl(\Xii'\Sgma\Xii\bigr)$}, by LIE and \ref{item:xu}.\ref{item:het}. The limit in probability \ref{item:V} and assumption \ref{item:mom}.\ref{item:mom_Adistr} are the two conditions that satisfy  the  \emph{Multivariate Central Limit Theorem} (\emph{MCLT}) for \emph{inid} processes  [\textsc{thm 6.16} in \citet[p.189]{hansen2019}]. Therefore, $N^{-1/2}\,\sum_{i=1}^N\Xii'\uii \overset{d}{\to}\N \bigl(\bm{0}, \Vv\bigr)$ as $N\to\infty$. 
%blocks A&B
\emph{Slutsky's Theorem} [\textsc{thm 6.22.2} in \citet[p.193]{hansen2019}] yields the result $\sqrt{N}\bigl(\bfen - \bm{\beta}\bigr) \overset{d}{\to} \N\bigl(\bm{0},\SSxx\inv \Vv\SSxx\inv\bigr)$, where $\SSxx\equiv\E\bigl(\Xii'\Xii\bigr)$. \textsc{thm 6.19} [\citet[p.192]{hansen2019}]  ensures that the above limits hold for any monotonic transformation of the data, e.g., the within-group transformation.

\section{Estimation of the Asymptotic Variance}

\par \red{Cattaneo 2018}
Given the above results under the model assumptions we made, the approximate distribution of the estimator of  $\bm{\beta}$ for large but finite samples is
\begin{equation}
\bfen\distas{a} \N(\bm{\beta}, N\inv\SSxx\inv\Vv \SSxx\inv),
 \end{equation}
 \noindent where the limiting matrices $\SSxx$ and  $\Vv$ need to be estimated, and  so does the average variance-covariance matrix $\bVn$.  While $\SSxx$ is straightforwardly estimated by $\Sxx = N\inv \sum_{i=1}^N \Xii'\Xii$, the estimation  of the average variance-covariance matrix needs further discussion.
 As pointed out by \mbox{\citet{white1980}}, a computationally feasible practice consists in estimating each expectation, $\Vi=\E\bigl(\Xii'\Sgma\Xii\bigr)$, individually. A plausible estimator of $\bVn$ would have been $ N\inv \sum_{i=1}^N\Xii'\uii\uii'\Xii$ if the error term were known. As it is unobserved, a plausible  consistent estimator of the  variance-covariance matrix is, therefore, $\Vh= N\inv \sum_{i=1}^N\Xii'\vi\vi'\Xii$, where $\vi=\Mi\inv\tui$ are the transformed regression residuals while the choice of $\Mi$ differs across the different covariance matrix estimators and \mbox{$\tui =\yi - \Xii\bfe$}.  Define $\tui = \resi$ to simplify the notation. The variance-covariance matrix  takes the familiar \emph{``sandwich-like''} formula of \mbox{\citeapos{arellano1987}} estimator when the transformed residuals equalise the residuals from the regression, i.e., $\vi=\resi$. Other functional forms of the transformed residuals will be presented in Section~\ref{sec:estimators}.
 \par Consistency of the variance-covariance matrix $\Vh$ with transformed residuals is proved under fixed $T$.   Let $\Sgmahat=\vi\vi'$, from \citeapos{white1980} general result and  the above model assumptions it follows that $\big\|\Vh-\bVn\big\|\overset{p}{\to}\bm{0}$  and, hence,  $\big\|N\inv\sum_i\Sgmahat-\bSgma\big\|\overset{p}{\to}\bm{0}$, for all $i=1,\dots,N$, as $N\to\infty$ and keeping $T$ fixed. 
%The estimator of variance of form $\Vh$ mirrors the EHW estimator used for robust inference in cross-sectional models, and its first formularisation has been suggested by \citet{arellano1987} following \mbox{\citet[Ch.6]{white1984}}.  
 \par Computationally, statistical softwares, e.g., \textsc{stata}, use a finite-sample modification of the conventional (i.e., \citeapos{arellano1987}) variance-covariance matrix  multiplying $N\inv\sum_{i=1}^N \Xii' \resi \resi'\Xii$ by the correction factor \mbox{$c=\frac{n-1}{n-k}\cdot\frac{N}{N-1}$}, where $n=N\cdot T$  for one-way clustering in panel data, otherwise cluster-robust standard error turn out to be downward biased  \citep{arellano1987, bertrand2004, cameron2011}. An extension of  \citeapos{arellano1987} estimator  with multiple-way clustering is provided in \citet{cameron2011}.  Whilst the cross-sectional literature on HC estimators offers a wide range of sophisticated formulae for the variance-covariance matrices with alternative predicted residuals in place of regression residuals, no alternatives to the \citeapos{arellano1987} estimator have been yet given for the panel data setting other than bootstrap and jackknife methods. In the next section, we  present a battery of HC estimators for panel data that are constructed with different functional forms of the predicted residuals.



